Optimizing Indoor RIS-Aided Physical-Layer Security: A Codebook-Generation Methodology and Measurement-Based Analysis

Sixth-Generation (6G) wireless networks aim to support innovative Internet-of-Things (IoT) applications that demand faster and more secure data transmission. While higher Open Systems Interconnection (OSI) layers employ measures like encryption and secure protocols to address data security, Physical-Layer Security (PLS) focuses on preventing information leakage to EavesDroppers (EDs) and mitigating the effects of jammers and spoofing attacks. In this context, the emerging technology of Reconfigurable Intelligent Surfaces (RISs) can play an instrumental role, enhancing PLS by intelligently reflecting electromagnetic waves to benefit Legitimate Users (LUs) while obstructing EDs. This paper presents practical indoor measurements to evaluate the capability of an RIS to enhance PLS, focusing on a varactor-based RIS technology designed for the FR1 band at 3.55 GHz. A comparative analysis of state-of-the-art RIS-aided secrecy optimization algorithms together with a novel approach designed in this paper, which relies on a newly generated RIS phase configuration codebook, highlight the potential of RISs to improve both data rates for LUs as well as secrecy against EDs in real-world indoor multipath environments. The results also demonstrate the frequency selectivity of the RIS, proviging practical insights on the optimization of the technology.

==> Radiation_Pattern_configs.tex <==
\begin{tikzpicture}
\begin{axis}[
    %title={Secrecy Rate \emph{vs.} Transmit Power ($N_0 = -165$~dBm)},
    xlabel={Angle ($\degree$)},
    ylabel={Received Power Pattern (dB)},
    xmin=0, xmax=33,
    ymin=-86, ymax=-67,
    xtick={0,15,30},
    %xticklabels={$0$,15,30,45},
    ytick={-67,-69,-71,-73,-75,-77,-79,-81,-83,-85},
    legend pos= north west, %north west
    ymajorgrids=true,
    yminorgrids=true,
    minor y tick num=2,
    grid style=dashed,
    legend columns=1,
    width=\columnwidth,
    height=7cm, 
legend style={%at={(1.1,1.02)},
    %%at={(0,-0.15)},
      nodes = { 
            % text width=1.5cm,  
            % anchor=base,
            % text depth=,
            scale=0.6,         %%
            transform shape},  %%
    legend cell align=left, 
    align=left, draw=white!15!black}
]

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (0,-78.42)(15,-81.71)(30,-83.87)%(45,-74.9716)
    };
    \addlegendentry{RIS-config. 1}
\addplot[
    color=green,
    mark=square
    ]
    coordinates {
    (0,-79.61)(15,-81.53)(30,-82.63)%(45,-74.0232)
    };
    \addlegendentry{RIS-config. 2}
    \addplot[
    color=red,
    mark=square
    ]
    coordinates {
    (0,-78.85)(15,-80.28)(30,-82.54)%(45,-83.0374)
    };
    \addlegendentry{RIS-config. 3}
    \addplot[
    color=blue,
    mark=triangle
    ]
    coordinates {
    (0,-81.98)(15,-69.03)(30,-78.8527)%(45,-69.0269)
    };
    \addlegendentry{RIS-config. 4}
    \addplot[
    color=green,
    mark=triangle,
    ]
    coordinates {
    (0,-83.76)(15,-71.43)(30,-82.22)%(45,-69.0269)
    };
    \addlegendentry{RIS-config. 5}
    \addplot[
    color=red,
    mark=triangle
    ]
    coordinates {
    (0,-82.79)(15,-72.22)(30,-78.8527)%(45,-69.0269)
    };
    \addlegendentry{RIS-config. 6}
    \addplot[
    color=blue,
    mark=diamond,
    ]
    coordinates {
    (0,-84.81)(15,-79.6109)(30,-78.8527)(45,-69.0269)
    };
    \addlegendentry{RIS-config. 7}
    \addplot[
    color=green,
    mark=diamond,
    ]
    coordinates {
    (0,-88.72)(15,-79.6109)(30,-78.8527)(45,-69.0269)
    };
    \addlegendentry{RIS-config. 8}
    \addplot[
    color=red,
    mark=diamond
    ]
    coordinates {
    (0,-84.74)(15,-79.6109)(30,-78.8527)(45,-69.0269)
    };
    \addlegendentry{RIS-config. 9}
\end{axis}
\end{tikzpicture}



\begin{comment}
    \begin{tikzpicture}
\begin{axis}[
    %title={Secrecy Rate \emph{vs.} Transmit Power ($N_0 = -165$~dBm)},
    xlabel={Angle ($\degree$)},
    ylabel={Received Power Pattern (dB)},
    xmin=0, xmax=3350,
    ymin=-86, ymax=-71,
    xtick={0,15,30,45},
    %xticklabels={$0$,15,30,45},
    ytick={-71,-73,-75,-77,-79,-81,-83,-85},
    legend pos= north west, %north west
    ymajorgrids=true,
    yminorgrids=true,
    minor y tick num=2,
    grid style=dashed,
    legend columns=1,
    width=\columnwidth,
    height=7cm, 
legend style={%at={(1.1,1.02)},
    %%at={(0,-0.15)},
      nodes = { 
            % text width=1.5cm,  
            % anchor=base,
            % text depth=,
            scale=0.6,         %%
            transform shape},  %%
    legend cell align=left, 
    align=left, draw=white!15!black}
]

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (0,-78.421071)(15,-71.71545)(30,-80.87664)%(45,-74.9716)
    };
    \addlegendentry{RIS-config. 1}
\addplot[
    color=green,
    mark=square
    ]
    coordinates {
    (0,-798.613937)(15,-810.52321)(30,-820.65393)%(45,-74.0232)
    };
    \addlegendentry{RIS-config. 2}
    \addplot[
    color=red,
    mark=square
    ]
    coordinates {%-77.1842
    (0,-78.8527)(15,-780.285815)(30,-820.73554)%(45,-83.0374)
    };
    \addlegendentry{RIS-config. 3}
    \addplot[
    color=blue,
    mark=triangle
    ]
    coordinates {
    (0,-84.017)(15,-79.6109)(30,-78.8527)(45,-69.0269)
    };
    \addlegendentry{RIS-config. 4}
    \addplot[
    color=green,
    mark=triangle,
    ]
    coordinates {
    (0,-83.76)(15,-79.6109)(30,-78.8527)(45,-69.0269)
    };
    \addlegendentry{RIS-config. 5}
    \addplot[
    color=red,
    mark=triangle
    ]
    coordinates {
    (0,-82.79)(15,-79.6109)(30,-78.8527)(45,-69.0269)
    };
    \addlegendentry{RIS-config. 6}
    \addplot[
    color=blue,
    mark=diamond,
    ]
    coordinates {
    (0,-84.81)(15,-79.6109)(30,-78.8527)(45,-69.0269)
    };
    \addlegendentry{RIS-config. 7}
    \addplot[
    color=green,
    mark=diamond,
    ]
    coordinates {
    (0,-88.72)(15,-79.6109)(30,-78.8527)(45,-69.0269)
    };
    \addlegendentry{RIS-config. 8}
    \addplot[
    color=red,
    mark=diamond
    ]
    coordinates {
    (0,-84.74)(15,-79.6109)(30,-78.8527)(45,-69.0269)
    };
    \addlegendentry{RIS-config. 9}
\end{axis}
\end{tikzpicture}
\end{comment}

==> mycompress.tex <==
\setlength{\textfloatsep}{-5pt plus 3pt minus 2.0pt}		% space between last top float or first bottom float and the text
\setlength{\floatsep}{0pt plus 0pt minus 2.0pt}			% space left between floats
\setlength{\dblfloatsep}{-1pt plus 0pt minus 3.0pt}			% space left between floats
\setlength{\dbltextfloatsep}{-1pt plus 0pt minus 3.0pt}			% space left between floats
\setlength{\abovecaptionskip}{0pt plus 0pt minus 10pt}	% space above caption
\setlength{\belowcaptionskip}{0pt plus 0pt minus 3pt}	% space below caption
\setlength{\abovedisplayskip}{1pt plus 1pt minus 2pt}	% space before maths
\setlength{\belowdisplayskip}{1pt plus 1pt minus 2pt}	% space after maths

\renewcommand{\topfraction}{0.90}
\renewcommand{\bottomfraction}{0.90}
\renewcommand{\floatpagefraction}{0.9}
\renewcommand{\textfraction}{0.02}
%extra compression with title spacings

\usepackage{titlesec}
\titlespacing*{\section}{0pt}{0pt plus 0pt minus 0pt}{0pt plus 1pt minus 2pt}
\titlespacing{\subsection}{0pt}{1pt plus 0pt minus 1pt}{0pt plus 0pt minus 1pt}
\titlespacing{\subsubsection}{0pt}{1pt plus 0pt minus 12pt}{1pt}


==> techniques_legend.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=2.083in,
height=2.083in,
at={(0.26in,0.26in)},
scale only axis,
xmin=-0.1,
xmax=1.1,
ymin=-0.1,
ymax=1.1,
axis line style={draw=none},
ticks=none,
title={},
axis x line*=bottom,
axis y line*=left
]

\addplot[area legend, line width=1.0pt, draw=black, fill=white, forget plot]
table[row sep=crcr] {%
x	y\\
0	1\\
1	1\\
0.7	0.6\\
0.3	0.6\\
}--cycle;

\addplot[area legend, line width=1.0pt, draw=black, fill=white, forget plot]
table[row sep=crcr] {%
x	y\\
1	1\\
1	0\\
0.6	0.2\\
0.7	0.6\\
}--cycle;

\addplot[area legend, line width=1.0pt, draw=black, fill=white, forget plot]
table[row sep=crcr] {%
x	y\\
0.6	0.2\\
1	0\\
0	0\\
0.4	0.2\\
}--cycle;

\addplot[area legend, line width=1.0pt, draw=black, fill=white, forget plot]
table[row sep=crcr] {%
x	y\\
0	1\\
0	0\\
0.4	0.2\\
0.3	0.6\\
}--cycle;

\addplot[area legend, line width=1.0pt, draw=black, fill=white, forget plot]
table[row sep=crcr] {%
x	y\\
0.3	0.6\\
0.7	0.6\\
0.6	0.2\\
0.4	0.2\\
}--cycle;
\node[centered, align=center, inner sep=0, font=\bfseries, rotate=180]
at (axis cs:0.5,0.75) {LU max.};
\node[centered, align=center, inner sep=0, font=\bfseries, rotate=180]
at (axis cs:0.825,0.45) {ED min.};
\node[centered, align=center, inner sep=0, font=\bfseries, rotate=180]
at (axis cs:0.5,0.15) {Alg. 1};
\node[centered, align=center, inner sep=0, font=\bfseries, rotate=180]
at (axis cs:0.175,0.45) {Alg.2};
\node[centered, align=center, inner sep=0, font=\bfseries, rotate=180]
at (axis cs:0.5,0.4) {Uniform\\Surface};
\end{axis}

\begin{axis}[%
width=2.604in,
height=2.604in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%
